Replacing the Irreplaceable: Fast Algorithms for Team Member Recommendation

In this paper, we study the problem of Team Member Replacement: given a team of people embedded in a social network working on the same task, find a good candidate who can fit in the team after one team member becomes unavailable. We conjecture that a good team member replacement should have good skill matching as well as good structure matching. We formulate this problem using the concept of graph kernel. To tackle the computational challenges, we propose a family of fast algorithms by (a) designing effective pruning strategies, and (b) exploring the smoothness between the existing and the new team structures. We conduct extensive experimental evaluations on real world datasets to demonstrate the effectiveness and efficiency. Our algorithms (a) perform significantly better than the alternative choices in terms of both precision and recall; and (b) scale sub-linearly.

==> 061vis.tex <==
We introduced a novel visualization technique to represent  authors' relationships and their expertises within one unique graph visualization. Particularly, in this visualization, the authors are shown as voronoi diagrams~\cite{du1999centroidal}. The authors' expertises are visualized as the voronoi cells inside the diagram, that is, each cell indicates a type of expertise.  We use different color hues to identify different expertise types and use the color saturations to encode the author's strength in that expertise type. For example, if KDD is represented in orange, a bright orange cell in a voronoi diagram means the author has a strong expertise in KDD. In opposite, a white cell indicates the author's lacking of the corresponding expertise. To facilitate visual comparison of different authors, we fix the position of these expertise cells across different diagrams so that, for example, KDD is always shown at the left side of the author diagrams.  These voronoi diagrams are connected by links indicating the authors' relationships. The strength of the relationship are presented by the line thickness.

